Faster Differentially Private Top-$k$ Selection: A Joint Exponential Mechanism with Pruning

We study the differentially private top-$k$ selection problem, aiming to identify a sequence of $k$ items with approximately the highest scores from $d$ items. Recent work by Gillenwater et al. (ICML '22) employs a direct sampling approach from the vast collection of $d^{\,\Theta(k)}$ possible length-$k$ sequences, showing superior empirical accuracy compared to previous pure or approximate differentially private methods. Their algorithm has a time and space complexity of $\tilde{O}(dk)$. In this paper, we present an improved algorithm with time and space complexity $O(d + k^2 / \epsilon \cdot \ln d)$, where $\epsilon$ denotes the privacy parameter. Experimental results show that our algorithm runs orders of magnitude faster than their approach, while achieving similar empirical accuracy.

==> auctual-counter-computation.tex <==
In this section, we show how to compute the $\cntUnified{r}{j}$'s efficiently. 
Recall that 
\begin{align}
    \cntUnified{r}{j} &\doteq \begin{cases}
        | \{ j' \in [d] : \hist\bracket{j'} \ge \hist_{(j)} - r \} |, & r < \tau. \\
        d,  & r = \tau.
    \end{cases} 
\end{align}

\begin{itemize}
    \item Group the indices of $\hist$ according to their values.
    In particular, for each $t \in \IntSet{0}{n}$, let 
    \begin{align*}
        \groupIndex\bracket{t} \doteq \{ i \in \cD : \hist[i] = t \}.
    \end{align*}
    The non-empty $\groupIndex\bracket{t}$'s constitute a partition of $\DataDomain$, and can be computed in $O(d)$ time with $O(d)$ space.

    \item Further, define the threshold 
    $
        \smallestTokSolnValue \doteq \hist[k] - \tau,
    $
    and let $t_1 > t_2 \cdots > t_m$ be the ordered index sequences of the set $\cT \doteq \set{t \in \IntSet{0}{n} : t > \smallestTokSolnValue \, \wedge \, \groupIndex\bracket{t} \neq \varnothing}$. 
    Identifying the elements in $\cT$ takes $O(d)$ time, and sorting these elements takes $O(m)$ time.
    Since $m < k + \tau$, the sequence can be computed in $O(d + (k + \tau) \log (k + \tau))$ time.

    \item Construct the sorted array of tuples: 
    \begin{align*}
        \sortedGroupArray
            \doteq \BigBracket{
                \paren{t_1, \groupIndex\bracket{t_1}}, 
                \ldots,
                \paren{t_m, \groupIndex\bracket{t_m}}
            }   
    \end{align*}
    This can also be constructed in $O(d)$ time.
    Then based on $\sortedGroupArray$, compute a prefix sum array
    \begin{align*}
        \prefixSumSortedGroupArray \doteq \PAREN{
            \prefixSumSortedGroupArray\bracket{1}, 
            \ldots,
            \prefixSumSortedGroupArray\bracket{m}
        },   
        \quad 
        \text{ s.t. } 
        \quad 
        \prefixSumSortedGroupArray\bracket{i} \doteq \sum_{j \in [i]} \card{\groupIndex\bracket{t_j}},
        \, 
        \quad \forall i \in [m].
    \end{align*} 

    \item For each $r \in \IntSet{0}{\tau - 1}$, $j \in [k]$, of interest is the position 
    \begin{align*}
        \posInSortedGroupArray{r}{j} \doteq \max \{i \in [m] : t_i \ge \hist_{(j)} - r \}.
    \end{align*}
    By definition, we have 
    $
        \cntUnified{r}{j} 
            = \sum_{i \in [\posInSortedGroupArray{r}{j}]} \card{\groupIndex\bracket{t_{i}}}
            = \prefixSumSortedGroupArray\BRACKET{\posInSortedGroupArray{r}{j}}. 
    $

    \item The $\posInSortedGroupArray{r}{j}$'s can be computed in $O(k \tau)$ time. 
    Clearly the $\posInSortedGroupArray{0}{j}$'s can be computed in $O(k)$ time. 
    We claim that for each $r \in \IntSet{1}{\tau - 1}$, $\posInSortedGroupArray{r}{j}$ can be computed in $O(1)$ time, once $\posInSortedGroupArray{r - 1}{j}$ is known:
    \begin{align}
        \posInSortedGroupArray{r}{j}
            \doteq \begin{cases}
                m, & \text{ if } \posInSortedGroupArray{r - 1}{j} = m \\
                1 + \posInSortedGroupArray{r - 1}{j}, & \text{ if } t_{1 + \posInSortedGroupArray{r - 1}{j}} \ge \hist[j] - r  \\
                \posInSortedGroupArray{r - 1}{j}, &  \text{ if } t_{1 + \posInSortedGroupArray{r - 1}{j}} < \hist[j] - r 
            \end{cases}
    \end{align}
    By definition, we have 
    \begin{align*}
        \posInSortedGroupArray{r}{j} \doteq \max \{i \in [m] : t_{i} \ge \hist_{(j)} - r \}, \quad 
        \posInSortedGroupArray{r - 1}{j} \doteq \max \{i \in [m] : t_{i} \ge \hist_{(j)} - r + 1\}.
    \end{align*}
    Then clearly we have $\posInSortedGroupArray{r}{j} \ge \posInSortedGroupArray{r - 1}{j}$. 
    But it also holds that $\posInSortedGroupArray{r}{j} \le \posInSortedGroupArray{r - 1}{j} + 1$. 
    The case is trivially true if $\posInSortedGroupArray{r - 1}{j} = m$ or $\posInSortedGroupArray{r - 1}{j} = m - 1$.
    Otherwise, since
    \begin{align*}
        t_{2 + \posInSortedGroupArray{r - 1}{j}} < t_{1 + \posInSortedGroupArray{r - 1}{j}} < t_{\posInSortedGroupArray{r - 1}{j}},
    \end{align*}
    if $t_{2 + \posInSortedGroupArray{r - 1}{j}} \ge \hist[j] - r$, then 
    \begin{align*}
        t_{1 + \posInSortedGroupArray{r - 1}{j}} \ge t_{2 + \posInSortedGroupArray{r - 1}{j}} + 1 \ge \hist[j] - r + 1,
    \end{align*}
    A contradiction.

    
\end{itemize}


==> reference-candidates.tex <==




@misc{MovieLens,
    title = {MovieLens 25M Dataset},
    author={Harper, F. Maxwell and Konstan, Joseph A.},
    howpublished = {\url{https://grouplens.org/datasets/movielens/25m/}},
    year={2019},
    note = {Accessed: 2024-05-10}
}


@article{HK15,
    title={\href{https://dl.acm.org/doi/10.1145/2827872}{The MovieLens Datasets: History and Context}},
    author={Harper, F. Maxwell and Konstan, Joseph A.},
    journal={Transactions on Interactive Intelligent Systems (TiiS)},
    year={2015}
}

